Microtubule Tracking in Electron Microscopy Volumes

We present a method for microtubule tracking in electron microscopy volumes. Our method first identifies a sparse set of voxels that likely belong to microtubules. Similar to prior work, we then enumerate potential edges between these voxels, which we represent in a candidate graph. Tracks of microtubules are found by selecting nodes and edges in the candidate graph by solving a constrained optimization problem incorporating biological priors on microtubule structure. For this, we present a novel integer linear programming formulation, which results in speed-ups of three orders of magnitude and an increase of 53% in accuracy compared to prior art (evaluated on three 1.2 x 4 x 4$\mu$m volumes of Drosophila neural tissue). We also propose a scheme to solve the optimization problem in a block-wise fashion, which allows distributed tracking and is necessary to process very large electron microscopy volumes. Finally, we release a benchmark dataset for microtubule tracking, here used for training, testing and validation, consisting of eight 30 x 1000 x 1000 voxel blocks (1.2 x 4 x 4$\mu$m) of densely annotated microtubules in the CREMI data set (https://github.com/nilsec/micron).

==> figures/results/block/block_timing.tikz.tex <==
\begin{tikzpicture}
    \begin{axis}[
        ymajorgrids=true,
        xmode=log,
        xmajorgrids=true,
        legend style={font=\tiny},
        legend image post style={scale=0.5},
        legend columns=1,
        legend pos=north west,
        xlabel={Block Size [voxel]},
        ylabel={ILP Solve Time/Block [s]},
        xticklabel style={font=\tiny,overlay},
        yticklabel style={font=\tiny,overlay},
        ylabel style={font=\tiny,overlay},
        xlabel style={font=\tiny,overlay}]

    \pgfplotstableread{data/block_timing.csv}\plotdataa
    %\pgfplotstableread{figures/results/timing/csv_data/G2_edges_constraints.csv}\plotdatab

    % the whole curve
    \addplot[color_2,thick,only marks,mark=*]
        table[x=Block_Size,y=t_ilp_block] {\plotdataa};

	\addplot[
      color_3!60!black,
      thick,
      mark=o,
      mark size=2,
      x filter/.code={
        \pgfplotstablegetelem{\coordindex}{validation}\of{\plotdataa}
        \ifnum\pgfplotsretval=1
        \else
        \def\pgfmathresult{}
        \fi
        }]
        table[x=Block_Size,y=t_ilp_block] {\plotdataa};

   %\addlegendentry{reformulated ILP}
    \end{axis}
\end{tikzpicture}

